Categorical Foundations of Formalized Condensed Mathematics

Condensed mathematics, developed by Clausen and Scholze over the last few years, proposes a generalization of topology with better categorical properties. It replaces the concept of a topological space by that of a condensed set, which can be defined as a sheaf for the coherent topology on a certain category of compact Hausdorff spaces. In this case, the sheaf condition has a fairly simple explicit description, which arises from studying the relationship between the coherent, regular and extensive topologies. In this paper, we establish this relationship under minimal assumptions on the category, going beyond the case of compact Hausdorff spaces. Along the way, we also provide a characterization of sheaves and covering sieves for these categories. All results in this paper have been fully formalized in the Lean proof assistant.

==> condensed.tex <==
Consider the following three categories, each containing the next as a full subcategory, and whose morphisms are continuous maps:
\begin{itemize}
    \item $\CompHaus$: the category of compact Hausdorff spaces.~\href{https://github.com/leanprover-community/mathlib4/blob/a5f752732b1765fb770fb10c1988725041193bcc/Mathlib/Topology/Category/CompHaus/Basic.lean#L38-L45}{\faExternalLink}
    \item $\Profinite$: the category of \emph{profinite} spaces, that we define, following \mathlib, as totally disconnected compact Hausdorff spaces. This category is equivalent to the pro-category of the category of finite sets (this last statement has not yet been formalized; see~\cite[Section 6]{dagur-itp-2024} for a more detailed discussion of the state of the category $\Profinite$ in \mathlib.).~\href{https://github.com/leanprover-community/mathlib4/blob/a5f752732b1765fb770fb10c1988725041193bcc/Mathlib/Topology/Category/Profinite/Basic.lean#L47-L51}{\faExternalLink}
    \item $\Stonean$: the category of \emph{Stonean} spaces, whose objects are extremally disconnected compact Hausdorff spaces~\href{https://github.com/leanprover-community/mathlib4/blob/a5f752732b1765fb770fb10c1988725041193bcc/Mathlib/Topology/Category/Stonean/Basic.lean#L41-L45}{\faExternalLink}. The condition of being extremally disconnected means that the closure of every open set is open. These spaces are precisely the projective objects in $\CompHaus$ (see~\cite[Theorem~2.5]{gleason} and \href{https://github.com/leanprover-community/mathlib4/blob/a5f752732b1765fb770fb10c1988725041193bcc/Mathlib/Topology/Category/Stonean/Basic.lean#L307-L316}{\faExternalLink}). It is easy to see that Stonean spaces are totally disconnected. A formalization of the fully faithful inclusion $\Stonean\subseteq\Profinite$ can be found in \href{https://github.com/leanprover-community/mathlib4/blob/a5f752732b1765fb770fb10c1988725041193bcc/Mathlib/Topology/Category/Stonean/Basic.lean#L125-L138}{\faExternalLink}.
\end{itemize}
We can equip all these categories with a Grothendieck topology called the \emph{coherent topology} (see~\S\ref{sec:preliminaries} for a general discussion about topologies on a category, and Definition~\ref{def:coherent coverage} for the precise definition of the coherent topology), and we prove general categorical results that together imply the following theorems, which characterize so-called \emph{condensed sets}.

\begin{theorem}
    \href{https://github.com/leanprover-community/mathlib4/blob/a5f752732b1765fb770fb10c1988725041193bcc/Mathlib/Condensed/Equivalence.lean}{\faExternalLink}
    The categories of sheaves for the coherent topology on $\CompHaus$, $\Profinite$, and $\Stonean$, are all equivalent.
\end{theorem}

\begin{definition}
    \href{https://github.com/leanprover-community/mathlib4/blob/a5f752732b1765fb770fb10c1988725041193bcc/Mathlib/Condensed/Basic.lean#L46-L47}{\faExternalLink}
    A \emph{condensed set} is a sheaf for the coherent topology on $\CompHaus$.
\end{definition}

\begin{remark}
    Equivalently, a condensed set is a sheaf for the coherent topology on $\Profinite$ or $\Stonean$.
\end{remark}

\begin{theorem}\label{thm:comphaus_sheaves}
    \href{https://github.com/leanprover-community/mathlib4/blob/a5f752732b1765fb770fb10c1988725041193bcc/Mathlib/CategoryTheory/Sites/Coherent/SheafComparison.lean#L235-L242}{\faExternalLink}
    Let $\C$ be either $\CompHaus$ or $\Profinite$. 
    A presheaf $X \colon \C^{\op} \to \Set$ is a sheaf for the coherent topology on $\C$ if and only if it satisfies the following two conditions:
    \begin{list_conditions}
        \item $X$ preserves finite products: in other words, for every finite family $(T_i)$ of object of $\C$, the natural map 
        \[
            X\Bigl(\coprod_i T_i\Bigr) \longrightarrow \prod_i X(T_i)    
        \]
        is a bijection.
        \item For every surjection $\pi \colon S \to T$ in $\C$, the diagram 
        \[\begin{tikzcd}
            {X(T)} & {X(S)} & {X(S \times_T S)}
            \arrow["{X(\pi)}", from=1-1, to=1-2]
            \arrow[shift left, from=1-2, to=1-3]
            \arrow[shift right, from=1-2, to=1-3]
        \end{tikzcd}\]
        is an equalizer \textup{(}the two parallel morphisms being given by the projections in the pullback\textup{)}. 
    \end{list_conditions}
\end{theorem}

A similar assertion holds true when $\C$ is $\Stonean$ as well, except that condition (2) must be modified slightly (e.g.~using $1$-hypercovers) due to the fact that $\Stonean$ does not have pullbacks.
However, this analogous condition turns out to be vacuously true in $\Stonean$, which is the content of the following theorem.

\begin{theorem}\label{thm:stonean_sheaves}
    \href{https://github.com/leanprover-community/mathlib4/blob/a5f752732b1765fb770fb10c1988725041193bcc/Mathlib/CategoryTheory/Sites/Coherent/SheafComparison.lean#L244-L248}{\faExternalLink}
    A presheaf $X \colon \Stonean^{\op} \to \Set$ is a sheaf for the coherent topology on $\Stonean$ if and only if it preserves finite products: in other words, for every finite family $(T_i)$ of object of $\C$, the natural map 
    \[
        X\Bigl(\coprod_i T_i\Bigr) \longrightarrow \prod_i X(T_i)    
    \]
    is a bijection.
\end{theorem}

Combining theorems~\ref{thm:condensed set equivalence} and~\ref{thm:stonean_sheaves}, we see that the category $\Stonean$ yields the simplest description of condensed sets, because the sheaf condition reduces to the simple condition of preserving finite products. At the same time, it is the most problematic of the three, in the sense that it barely has any limits and it does not have pullbacks in general --- and not even binary products. It is difficult to imagine its objects, examples of which mostly come from Stone--\Cech compactifications of discrete sets. The poor categorical properties of $\Stonean$ is one of the motivations to prove results in the high level of generality chosen the present paper.


==> lstlean.tex <==
% Listing style definition for the Lean Theorem Prover.
% Defined by Jeremy Avigad, 2015, by modifying Assia Mahboubi's SSR style.
% Unicode replacements taken from Olivier Verdier's unixode.sty

\lstdefinelanguage{lean} {

% % Anything between $ becomes LaTeX math mode
mathescape=false,
% Comments may or not include Latex commands
texcl=false,

% keywords, list taken from lean-syntax.el
morekeywords=[1]{
import, prelude, protected, private, noncomputable, definition, meta, renaming,
hiding, parameter, parameters, begin, constant, constants,
lemma, variable, variables, theory,
print, theorem, example,
open, as, export, override, axiom, axioms, inductive, with,
structure, record, universe, universes,
alias, help, precedence, reserve, declare_trace, add_key_equivalence,
match, infix, infixl, infixr, notation, postfix, prefix, instance,
reduce, check, end, this,
using, using_well_founded, namespace, section,
attribute, local, set_option, extends, include, omit, class,
raw, replacing,
calc, have, show, suffices, by, in, at, let, forall, Pi, fun,
exists, if, dif, then, else, assume, obtain, from, register_simp_ext, unless, break, continue,
mutual, do, def, run_cmd, const,
partial, mut, where, macro, syntax, deriving,
return, try, catch, for, macro_rules, declare_syntax_cat, abbrev},

% Sorts
morekeywords=[2]{Sort, Type, Prop},

% tactics, list taken from lean-syntax.el
morekeywords=[3]{
assumption,
apply, intro, intros, allGoals,
generalize, clear, revert, done, exact,
refine, repeat, cases, rewrite, rw,
simp, simp_all, contradiction,
constructor, injection,
induction,
},

% modifiers, taken from lean-syntax.el
% note: 'otherkeywords' is needed because these use a different symbol.
% this command doesn't allow us to specify a number -- they are put with [1]
% otherkeywords={
% [persistent], [notation], [visible], [instance], [trans_instance],
% [class], [parsing-only], [coercion], [unfold_full], [constructor],
% [reducible], [irreducible], [semireducible], [quasireducible], [wf],
% [whnf], [multiple_instances], [none], [decl], [declaration],
% [relation], [symm], [subst], [refl], [trans], [simp], [congr], [unify],
% [backward], [forward], [no_pattern], [begin_end], [tactic], [abbreviation],
% [reducible], [unfold], [alias], [eqv], [intro], [intro!], [elim], [grinder],
% [localrefinfo], [recursor]
% },

% Various symbols
literate=
{α}{{\ensuremath{\mathrm{\alpha}}}}1
{β}{{\ensuremath{\mathrm{\beta}}}}1
{γ}{{\ensuremath{\mathrm{\gamma}}}}1
{δ}{{\ensuremath{\mathrm{\delta}}}}1
{ε}{{\ensuremath{\mathrm{\varepsilon}}}}1
{ζ}{{\ensuremath{\mathrm{\zeta}}}}1
{η}{{\ensuremath{\mathrm{\eta}}}}1
{θ}{{\ensuremath{\mathrm{\theta}}}}1
{ι}{{\ensuremath{\mathrm{\iota}}}}1
{κ}{{\ensuremath{\mathrm{\kappa}}}}1
{μ}{{\ensuremath{\mathrm{\mu}}}}1
{ν}{{\ensuremath{\mathrm{\nu}}}}1
{ξ}{{\ensuremath{\mathrm{\xi}}}}1
{π}{{\ensuremath{\mathrm{\mathnormal{\pi}}}}}1
{ρ}{{\ensuremath{\mathrm{\rho}}}}1
{σ}{{\ensuremath{\mathrm{\sigma}}}}1
{τ}{{\ensuremath{\mathrm{\tau}}}}1
{φ}{{\ensuremath{\mathrm{\varphi}}}}1
{χ}{{\ensuremath{\mathrm{\chi}}}}1
{ψ}{{\ensuremath{\mathrm{\psi}}}}1
{ω}{{\ensuremath{\mathrm{\omega}}}}1

{Γ}{{\ensuremath{\mathrm{\Gamma}}}}1
{Δ}{{\ensuremath{\mathrm{\Delta}}}}1
{Θ}{{\ensuremath{\mathrm{\Theta}}}}1
{Λ}{{\ensuremath{\mathrm{\Lambda}}}}1
{Σ}{{\ensuremath{\mathrm{\Sigma}}}}1
{Φ}{{\ensuremath{\mathrm{\Phi}}}}1
{Ξ}{{\ensuremath{\mathrm{\Xi}}}}1
{Ψ}{{\ensuremath{\mathrm{\Psi}}}}1
{Ω}{{\ensuremath{\mathrm{\Omega}}}}1

{ℵ}{{\ensuremath{\aleph}}}1

{≤}{{\ensuremath{\leq}}}1
{≥}{{\ensuremath{\geq}}}1
{≠}{{\ensuremath{\neq}}}1
{≈}{{\ensuremath{\approx}}}1
{≡}{{\ensuremath{\equiv}}}1
{≃}{{\ensuremath{\simeq}}}1

{≤}{{\ensuremath{\leq}}}1
{≥}{{\ensuremath{\geq}}}1

{∂}{{\ensuremath{\partial}}}1
{∆}{{\ensuremath{\triangle}}}1 % or \laplace?

{∫}{{\ensuremath{\int}}}1
{∑}{{\ensuremath{\mathrm{\Sigma}}}}1
{Π}{{\ensuremath{\mathrm{\Pi}}}}1

{⊥}{{\ensuremath{\perp}}}1
{∞}{{\ensuremath{\infty}}}1
{∂}{{\ensuremath{\partial}}}1

{∓}{{\ensuremath{\mp}}}1
{±}{{\ensuremath{\pm}}}1
{×}{{\ensuremath{\times}}}1

{⊕}{{\ensuremath{\oplus}}}1
{⊗}{{\ensuremath{\otimes}}}1
{⊞}{{\ensuremath{\boxplus}}}1

{∇}{{\ensuremath{\nabla}}}1
{√}{{\ensuremath{\sqrt}}}1

{⬝}{{\ensuremath{\cdot}}}1
{•}{{\ensuremath{\cdot}}}1
{∘}{{\ensuremath{\circ}}}1

%{⁻}{{\ensuremath{^{\textup{\kern1pt\rule{2pt}{0.3pt}\kern-1pt}}}}}1
{⁻}{{\ensuremath{^{-}}}}1
{▸}{{\ensuremath{\blacktriangleright}}}1

{∧}{{\ensuremath{\wedge}}}1
{∨}{{\ensuremath{\vee}}}1
{¬}{{\ensuremath{\neg}}}1
{⊢}{{\ensuremath{\vdash}}}1

%{⟨}{{\ensuremath{\left\langle}}}1
%{⟩}{{\ensuremath{\right\rangle}}}1
{⟨}{{\ensuremath{\langle}}}1
{⟩}{{\ensuremath{\rangle}}}1

{↦}{{\ensuremath{\mapsto}}}1
{←}{{\ensuremath{\leftarrow}}}1
{<-}{{\ensuremath{\leftarrow}}}1
{→}{{\ensuremath{\rightarrow}}}1
{↔}{{\ensuremath{\leftrightarrow}}}1
{⇒}{{\ensuremath{\Rightarrow}}}1
{⟹}{{\ensuremath{\Longrightarrow}}}1
{⇐}{{\ensuremath{\Leftarrow}}}1
{⟸}{{\ensuremath{\Longleftarrow}}}1
{⥤}{{\ensuremath{\func}}}1
{⟶}{{\ensuremath{\longrightarrow}}}1
{≫}{{\ensuremath{\gg}}}1 %%TODO: correct (AT: I think it's correct now)
{⋙}{{\ensuremath{\ggg}}}1 %%TODO: correct (AT: I think it's correct now)

{∩}{{\ensuremath{\cap}}}1
{∪}{{\ensuremath{\cup}}}1
{⊂}{{\ensuremath{\subseteq}}}1
{⊆}{{\ensuremath{\subseteq}}}1
{⊄}{{\ensuremath{\nsubseteq}}}1
{⊈}{{\ensuremath{\nsubseteq}}}1
{⊃}{{\ensuremath{\supseteq}}}1
{⊇}{{\ensuremath{\supseteq}}}1
{⊅}{{\ensuremath{\nsupseteq}}}1
{⊉}{{\ensuremath{\nsupseteq}}}1
{∈}{{\ensuremath{\in}}}1
{∉}{{\ensuremath{\notin}}}1
{∋}{{\ensuremath{\ni}}}1
{∌}{{\ensuremath{\notni}}}1
{∅}{{\ensuremath{\emptyset}}}1

{∖}{{\ensuremath{\setminus}}}1
{†}{{\ensuremath{\dag}}}1

{ℕ}{{\ensuremath{\mathbb{N}}}}1
{ℤ}{{\ensuremath{\mathbb{Z}}}}1
{ℝ}{{\ensuremath{\mathbb{R}}}}1
{ℚ}{{\ensuremath{\mathbb{Q}}}}1
{ℂ}{{\ensuremath{\mathbb{C}}}}1
{⌞}{{\ensuremath{\llcorner}}}1
{⌟}{{\ensuremath{\lrcorner}}}1
{⦃}{{\ensuremath{\{\!|}}}1
{⦄}{{\ensuremath{|\!\}}}}1

{‖}{{\ensuremath{\|}}}1
{₁}{{\ensuremath{_1}}}1
{₂}{{\ensuremath{_2}}}1
{₃}{{\ensuremath{_3}}}1
{₄}{{\ensuremath{_4}}}1
{₅}{{\ensuremath{_5}}}1
{₆}{{\ensuremath{_6}}}1
{₇}{{\ensuremath{_7}}}1
{₈}{{\ensuremath{_8}}}1
{₉}{{\ensuremath{_9}}}1
{₀}{{\ensuremath{_0}}}1
{ᵢ}{{\ensuremath{_i}}}1
{ⱼ}{{\ensuremath{_j}}}1
{ₐ}{{\ensuremath{_a}}}1

{¹}{{\ensuremath{^1}}}1

{ₙ}{{\ensuremath{_n}}}1
{ₘ}{{\ensuremath{_m}}}1
{ₚ}{{\ensuremath{_p}}}1
{↑}{{\ensuremath{\uparrow}}}1
{↓}{{\ensuremath{\downarrow}}}1

{...}{{\ensuremath{\ldots}}}1
{·}{{\ensuremath{\cdot}}}1

{▸}{{\ensuremath{\triangleright}}}1

{Σ}{{\color{symbolcolor}\ensuremath{\Sigma}}}1
{⊤}{{\color{symbolcolor}\ensuremath{\Top}}}1
{Π}{{\color{symbolcolor}\ensuremath{\Pi}}}1
{∀}{{\color{symbolcolor}\ensuremath{\forall}}}1
{∃}{{\color{symbolcolor}\ensuremath{\exists}}}1
{λ}{{\color{symbolcolor}\ensuremath{\mathrm{\lambda}}}}1
{\$}{{\color{symbolcolor}\$}}1

{:=}{{\color{symbolcolor}:=}}1
{=}{{\color{symbolcolor}=}}1
{<|>}{{\color{symbolcolor}<|>}}1
{<\$>}{{\color{symbolcolor}<\$>}}1
{+}{{\color{symbolcolor}+}}1
{*}{{\color{symbolcolor}*}}1,

% Comments
%comment=[s][\itshape \color{commentcolor}]{/-}{-/},
morecomment=[s][\color{commentcolor}]{/-}{-/},
morecomment=[l][\itshape \color{commentcolor}]{--},

% Spaces are not displayed as a special character
showstringspaces=false,

% keep spaces
keepspaces=true,

% String delimiters
morestring=[b]",
morestring=[d],

% Size of tabulations
tabsize=3,

% Enables ASCII chars 128 to 255
extendedchars=true,

% Case sensitivity
sensitive=true,

% Automatic breaking of long lines
breaklines=true,
breakatwhitespace=true,

% Default style fors listingsred
basicstyle=\ttfamily,

% % Position of captions is bottom
% captionpos=b,

% Full flexible columns
columns=[l]fullflexible,


% Style for (listings') identifiers
identifierstyle={\ttfamily\color{black}},
% Note : highlighting of Coq identifiers is done through a new
% delimiter definition through an lstset at the beginning of the
% document. Don't know how to do better.

% Style for declaration keywords
keywordstyle=[1]{\ttfamily\color{keywordcolor}},

% Style for sorts
keywordstyle=[2]{\ttfamily\color{sortcolor}},

% Style for tactics keywords
keywordstyle=[3]{\ttfamily\color{tacticcolor}},

% Style for attributes
keywordstyle=[4]{\ttfamily\color{attributecolor}},

% Style for strings
stringstyle=\ttfamily,

% Style for comments
commentstyle={\ttfamily\footnotesize },

}

